Experimental Comparison of Global Motion Planning Algorithms for Wheeled Mobile Robots

Planning smooth and energy-efficient motions for wheeled mobile robots is a central task for applications ranging from autonomous driving to service and intralogistic robotics. Over the past decades, a wide variety of motion planners, steer functions and path-improvement techniques have been proposed for such non-holonomic systems. With the objective of comparing this large assortment of state-of-the-art motion-planning techniques, we introduce a novel open-source motion-planning benchmark for wheeled mobile robots, whose scenarios resemble real-world applications (such as navigating warehouses, moving in cluttered cities or parking), and propose metrics for planning efficiency and path quality. Our benchmark is easy to use and extend, and thus allows practitioners and researchers to evaluate new motion-planning algorithms, scenarios and metrics easily. We use our benchmark to highlight the strengths and weaknesses of several common state-of-the-art motion planners and provide recommendations on when they should be used.

==> table-parking1.tex <==
\begin{tabular}{l*{5}{S[table-format=4.2(6)]}}
\toprule
\bf Planner & \mcc{Solutions Found} & \mcc{Computation Time [s]} & \mcc{Path Length} & \mcc{Maximum Curvature} & \mcc{Cusps} \\\midrule
\rowlabel{\textbf{Steer function: \texttt{Reeds-Shepp}} (\SI{0.2}{\minute} time limit)}
\\RRT                                      & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.02 \pm 0.00&
	{\databar{1.00}}	20.29 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	6%
\\
EST                                      & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.01 \pm 0.00&
	{\databar{1.00}}	23.39 \pm 0.00&
	{\databar{1.00}}	4.17 \pm 0.00&
	{\databar{1.00}}	6%
\\
RRT\#                                    & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.01 \pm 0.00&
	{\databar{1.00}}	15.83 \pm 0.00&
	{\databar{1.00}}	5.93 \pm 0.00&
	{\databar{1.00}}	6%
\\
kBITstar                                 & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.03 \pm 0.00&
	{\databar{1.00}}	14.55 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	9%
\\
BFMT                                     & %
	{\databar{1.00}}	1&
	{\databar{0.04}}	0.65 \pm 0.00&
	{\databar{1.00}}	11.41 \pm 0.00&
	{\databar{0.26}}	0.26 \pm 0.00&
	{\databar{1.00}}	5%
\\
KPIECE1                                  & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.04 \pm 0.00&
	{\databar{1.00}}	52.25 \pm 0.00&
	{\databar{1.00}}	3.87 \pm 0.00&
	{\databar{1.00}}	19%
\\
SORRTstar                                & %
	{\databar{1.00}}	1&
	{\databar{0.03}}	0.45 \pm 0.00&
	{\databar{1.00}}	13.18 \pm 0.00&
	{\databar{0.66}}	0.66 \pm 0.00&
	{\databar{1.00}}	7%
\\
RRTstar                                  & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.02 \pm 0.00&
	{\databar{1.00}}	15.83 \pm 0.00&
	{\databar{1.00}}	5.93 \pm 0.00&
	{\databar{1.00}}	6%
\\
SST                                      & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.02 \pm 0.00&
	{\databar{1.00}}	14.17 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	4%
\\
InformedRRTstar                          & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.01 \pm 0.00&
	{\databar{1.00}}	15.31 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	4%
\\
CForest                                  & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.04 \pm 0.00&
	{\databar{1.00}}	16.92 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	4%
\\
PRMstar                                  & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.03 \pm 0.00&
	{\databar{1.00}}	19.97 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	3%
\\
SPARS                                    & %
	{\databar{1.00}}	1&
	{\databar{0.01}}	0.12 \pm 0.00&
	{\databar{1.00}}	22.89 \pm 0.00&
	{\databar{0.39}}	0.39 \pm 0.00&
	{\databar{1.00}}	7%
\\
SPARStwo                                 & %
	{\databar{1.00}}	1&
	{\databar{0.27}}	4.12 \pm 0.00&
	{\databar{1.00}}	22.95 \pm 0.00&
	{\databar{1.00}}	4.03 \pm 0.00&
	{\databar{1.00}}	9%
\\
PDST                                     & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.07 \pm 0.00&
	{\databar{1.00}}	17.32 \pm 0.00&
	{\databar{1.00}}	4.27 \pm 0.00&
	{\databar{1.00}}	4%
\\
PRM                                      & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.04 \pm 0.00&
	{\databar{1.00}}	19.97 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	3%
\\
\rowlabel{\textbf{Steer function: \texttt{Dubins}} (\SI{0.8}{\minute} time limit)}
\\SPARS                                    & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
PRMstar                                  & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.14 \pm 0.00&
	{\databar{1.00}}	59.15 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	3%
\\
kBITstar                                 & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
RRT                                      & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.07 \pm 0.00&
	{\databar{1.00}}	27.44 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	4%
\\
KPIECE1                                  & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.03 \pm 0.00&
	{\databar{1.00}}	27.06 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	2%
\\
SORRTstar                                & %
	{\databar{1.00}}	1&
	{\databar{0.01}}	0.35 \pm 0.00&
	{\databar{1.00}}	24.28 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	2%
\\
SST                                      & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.01 \pm 0.00&
	{\databar{1.00}}	23.74 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	2%
\\
RRT\#                                    & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.09 \pm 0.00&
	{\databar{1.00}}	27.44 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	4%
\\
SPARStwo                                 & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
InformedRRTstar                          & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.11 \pm 0.00&
	{\databar{1.00}}	31.33 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	6%
\\
EST                                      & %
	{\databar{1.00}}	1&
	{\databar{0.76}}	33.98 \pm 0.00&
	{\databar{1.00}}	154.61 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	7%
\\
BFMT                                     & %
	{\databar{1.00}}	1&
	{\databar{0.64}}	28.93 \pm 0.00&
	{\databar{1.00}}	51.95 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	3%
\\
RRTstar                                  & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.09 \pm 0.00&
	{\databar{1.00}}	23.79 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	2%
\\
PRM                                      & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.13 \pm 0.00&
	{\databar{1.00}}	59.15 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	3%
\\
PDST                                     & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.22 \pm 0.00&
	{\databar{1.00}}	82.70 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	4%
\\
CForest                                  & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.21 \pm 0.00&
	{\databar{1.00}}	25.25 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	4%
\\
\rowlabel{\textbf{Steer function: \texttt{POSQ}} (\SI{2.0}{\minute} time limit)}
\\kBITstar                                 & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.04 \pm 0.00&
	{\databar{1.00}}	1.11 \pm 0.00&
	{\databar{0.86}}	0.86 \pm 0.00&
	{\databar{1.00}}	1%
\\
SPARStwo                                 & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.04 \pm 0.00&
	{\databar{1.00}}	1.18 \pm 0.00&
	{\databar{0.50}}	0.50 \pm 0.00&
	{\databar{1.00}}	11%
\\
SST                                      & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
RRTstar                                  & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.06 \pm 0.00&
	{\databar{1.00}}	1.46 \pm 0.00&
	{\databar{1.00}}	1.90 \pm 0.00&
	{\databar{1.00}}	6%
\\
PRM                                      & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.05 \pm 0.00&
	{\databar{1.00}}	1.28 \pm 0.00&
	{\databar{1.00}}	1.43 \pm 0.00&
	{\databar{1.00}}	17%
\\
CForest                                  & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.11 \pm 0.00&
	{\databar{1.00}}	1.15 \pm 0.00&
	{\databar{1.00}}	1.06 \pm 0.00&
	{\databar{1.00}}	17%
\\
KPIECE1                                  & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.11 \pm 0.00&
	{\databar{1.00}}	2.21 \pm 0.00&
	{\databar{1.00}}	3.64 \pm 0.00&
	{\databar{1.00}}	18%
\\
BFMT                                     & %
	{\databar{1.00}}	1&
	{\databar{0.13}}	15.88 \pm 0.00&
	{\databar{1.00}}	1.34 \pm 0.00&
	{\databar{0.57}}	0.57 \pm 0.00&
	{\databar{1.00}}	7%
\\
RRT                                      & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.04 \pm 0.00&
	{\databar{1.00}}	1.46 \pm 0.00&
	{\databar{1.00}}	1.90 \pm 0.00&
	{\databar{1.00}}	6%
\\
EST                                      & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.01 \pm 0.00&
	{\databar{1.00}}	1.64 \pm 0.00&
	{\databar{1.00}}	1.56 \pm 0.00&
	{\databar{1.00}}	8%
\\
SPARS                                    & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.09 \pm 0.00&
	{\databar{1.00}}	1.59 \pm 0.00&
	{\databar{1.00}}	1.26 \pm 0.00&
	{\databar{1.00}}	1%
\\
PRMstar                                  & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.20 \pm 0.00&
	{\databar{1.00}}	1.67 \pm 0.00&
	{\databar{0.91}}	0.91 \pm 0.00&
	{\databar{1.00}}	5%
\\
RRT\#                                    & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.04 \pm 0.00&
	{\databar{1.00}}	1.46 \pm 0.00&
	{\databar{1.00}}	1.90 \pm 0.00&
	{\databar{1.00}}	6%
\\
InformedRRTstar                          & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.02 \pm 0.00&
	{\databar{1.00}}	1.18 \pm 0.00&
	{\databar{0.50}}	0.50 \pm 0.00&
	{\databar{1.00}}	11%
\\
SORRTstar                                & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.08 \pm 0.00&
	{\databar{1.00}}	1.23 \pm 0.00&
	{\databar{0.63}}	0.63 \pm 0.00&
	{\databar{1.00}}	1%
\\
PDST                                     & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.03 \pm 0.00&
	{\databar{1.00}}	1.21 \pm 0.00&
	{\databar{0.59}}	0.59 \pm 0.00&
	{\databar{1.00}}	10%
\\
\rowlabel{\textbf{Steer function: \texttt{CC Reeds-Shepp}} (\SI{1.5}{\minute} time limit)}
\\EST                                      & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.05 \pm 0.00&
	{\databar{1.00}}	342.99 \pm 0.00&
	{\databar{0.20}}	0.20 \pm 0.00&
	{\databar{1.00}}	2%
\\
SST                                      & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.30 \pm 0.00&
	{\databar{1.00}}	288.15 \pm 0.00&
	{\databar{1.00}}	2.18 \pm 0.00&
	{\databar{1.00}}	9%
\\
kBITstar                                 & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.03 \pm 0.00&
	{\databar{1.00}}	342.99 \pm 0.00&
	{\databar{0.20}}	0.20 \pm 0.00&
	{\databar{1.00}}	2%
\\
SORRTstar                                & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.39 \pm 0.00&
	{\databar{1.00}}	246.72 \pm 0.00&
	{\databar{1.00}}	3.23 \pm 0.00&
	{\databar{1.00}}	11%
\\
PRMstar                                  & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.07 \pm 0.00&
	{\databar{1.00}}	342.99 \pm 0.00&
	{\databar{0.20}}	0.20 \pm 0.00&
	{\databar{1.00}}	2%
\\
RRT\#                                    & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.37 \pm 0.00&
	{\databar{1.00}}	329.18 \pm 0.00&
	{\databar{1.00}}	4.75 \pm 0.00&
	{\databar{1.00}}	8%
\\
PDST                                     & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.35 \pm 0.00&
	{\databar{1.00}}	332.35 \pm 0.00&
	{\databar{0.20}}	0.20 \pm 0.00&
	{\databar{1.00}}	4%
\\
InformedRRTstar                          & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.33 \pm 0.00&
	{\databar{1.00}}	280.21 \pm 0.00&
	{\databar{1.00}}	1.35 \pm 0.00&
	{\databar{1.00}}	7%
\\
BFMT                                     & %
	{\databar{1.00}}	1&
	{\databar{0.31}}	28.01 \pm 0.00&
	{\databar{1.00}}	300.10 \pm 0.00&
	{\databar{0.20}}	0.20 \pm 0.00&
	{\databar{1.00}}	3%
\\
PRM                                      & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.09 \pm 0.00&
	{\databar{1.00}}	342.99 \pm 0.00&
	{\databar{0.20}}	0.20 \pm 0.00&
	{\databar{1.00}}	2%
\\
RRT                                      & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.40 \pm 0.00&
	{\databar{1.00}}	329.18 \pm 0.00&
	{\databar{1.00}}	4.75 \pm 0.00&
	{\databar{1.00}}	8%
\\
RRTstar                                  & %
	{\databar{1.00}}	1&
	{\databar{0.01}}	0.46 \pm 0.00&
	{\databar{1.00}}	329.18 \pm 0.00&
	{\databar{1.00}}	4.75 \pm 0.00&
	{\databar{1.00}}	8%
\\
KPIECE1                                  & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.19 \pm 0.00&
	{\databar{1.00}}	289.22 \pm 0.00&
	{\databar{0.91}}	0.91 \pm 0.00&
	{\databar{1.00}}	3%
\\
SPARS                                    & %
	{\databar{1.00}}	1&
	{\databar{0.13}}	11.51 \pm 0.00&
	{\databar{1.00}}	304.37 \pm 0.00&
	{\databar{1.00}}	1.64 \pm 0.00&
	{\databar{1.00}}	11%
\\
SPARStwo                                 & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
CForest                                  & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.37 \pm 0.00&
	{\databar{1.00}}	296.11 \pm 0.00&
	{\databar{0.20}}	0.20 \pm 0.00&
	{\databar{1.00}}	5%
\\
\bottomrule
\end{tabular}

==> table-parking2.tex <==
\begin{tabular}{l*{5}{S[table-format=4.2(6)]}}
\toprule
\bf Planner & \mcc{Solutions Found} & \mcc{Computation Time [s]} & \mcc{Path Length} & \mcc{Maximum Curvature} & \mcc{Cusps} \\\midrule
\rowlabel{\textbf{Steer function: \texttt{Reeds-Shepp}} (\SI{0.2}{\minute} time limit)}
\\EST                                      & %
	{\databar{1.00}}	1&
	{\databar{0.02}}	0.28 \pm 0.00&
	{\databar{1.00}}	42.31 \pm 0.00&
	{\databar{1.00}}	4.34 \pm 0.00&
	{\databar{1.00}}	17%
\\
RRT\#                                    & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.02 \pm 0.00&
	{\databar{1.00}}	21.50 \pm 0.00&
	{\databar{1.00}}	4.44 \pm 0.00&
	{\databar{1.00}}	3%
\\
KPIECE1                                  & %
	{\databar{1.00}}	1&
	{\databar{0.01}}	0.11 \pm 0.00&
	{\databar{1.00}}	56.57 \pm 0.00&
	{\databar{1.00}}	3.46 \pm 0.00&
	{\databar{1.00}}	24%
\\
PRM                                      & %
	{\databar{1.00}}	1&
	{\databar{0.01}}	0.08 \pm 0.00&
	{\databar{1.00}}	22.08 \pm 0.00&
	{\databar{1.00}}	1.81 \pm 0.00&
	{\databar{1.00}}	5%
\\
RRTstar                                  & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.02 \pm 0.00&
	{\databar{1.00}}	21.50 \pm 0.00&
	{\databar{1.00}}	4.44 \pm 0.00&
	{\databar{1.00}}	3%
\\
SORRTstar                                & %
	{\databar{1.00}}	1&
	{\databar{0.22}}	3.25 \pm 0.00&
	{\databar{1.00}}	19.07 \pm 0.00&
	{\databar{1.00}}	4.07 \pm 0.00&
	{\databar{1.00}}	1%
\\
kBITstar                                 & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.06 \pm 0.00&
	{\databar{1.00}}	19.94 \pm 0.00&
	{\databar{1.00}}	4.91 \pm 0.00&
	{\databar{1.00}}	3%
\\
InformedRRTstar                          & %
	{\databar{1.00}}	1&
	{\databar{0.01}}	0.09 \pm 0.00&
	{\databar{1.00}}	24.52 \pm 0.00&
	{\databar{1.00}}	1.71 \pm 0.00&
	{\databar{1.00}}	5%
\\
CForest                                  & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.03 \pm 0.00&
	{\databar{1.00}}	18.60 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	1%
\\
Theta${}^*$                              & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
BFMT                                     & %
	{\databar{1.00}}	1&
	{\databar{0.08}}	1.22 \pm 0.00&
	{\databar{1.00}}	19.23 \pm 0.00&
	{\databar{1.00}}	2.86 \pm 0.00&
	{\databar{1.00}}	3%
\\
PRMstar                                  & %
	{\databar{1.00}}	1&
	{\databar{0.01}}	0.09 \pm 0.00&
	{\databar{1.00}}	22.08 \pm 0.00&
	{\databar{1.00}}	1.81 \pm 0.00&
	{\databar{1.00}}	5%
\\
RRT                                      & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.02 \pm 0.00&
	{\databar{1.00}}	21.50 \pm 0.00&
	{\databar{1.00}}	4.44 \pm 0.00&
	{\databar{1.00}}	3%
\\
PDST                                     & %
	{\databar{1.00}}	1&
	{\databar{0.02}}	0.28 \pm 0.00&
	{\databar{1.00}}	21.77 \pm 0.00&
	{\databar{1.00}}	1.74 \pm 0.00&
	{\databar{1.00}}	5%
\\
SPARStwo                                 & %
	{\databar{1.00}}	1&
	{\databar{0.45}}	6.77 \pm 0.00&
	{\databar{1.00}}	22.45 \pm 0.00&
	{\databar{0.37}}	0.37 \pm 0.00&
	{\databar{1.00}}	7%
\\
SPARS                                    & %
	{\databar{1.00}}	1&
	{\databar{0.09}}	1.29 \pm 0.00&
	{\databar{1.00}}	33.97 \pm 0.00&
	{\databar{1.00}}	4.81 \pm 0.00&
	{\databar{1.00}}	11%
\\
SST                                      & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	15.00 \pm 0.00&
	{\databar{1.00}}	22.27 \pm 0.00&
	{\databar{1.00}}	4.45 \pm 0.00&
	{\databar{1.00}}	3%
\\
\rowlabel{\textbf{Steer function: \texttt{Dubins}} (\SI{0.8}{\minute} time limit)}
\\PRMstar                                  & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.01 \pm 0.00&
	{\databar{1.00}}	35.69 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	1%
\\
PDST                                     & %
	{\databar{1.00}}	1&
	{\databar{0.01}}	0.25 \pm 0.00&
	{\databar{1.00}}	72.85 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	4%
\\
kBITstar                                 & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
InformedRRTstar                          & %
	{\databar{1.00}}	1&
	{\databar{0.02}}	1.01 \pm 0.00&
	{\databar{1.00}}	39.54 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	3%
\\
SPARS                                    & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
SORRTstar                                & %
	{\databar{1.00}}	1&
	{\databar{0.05}}	2.21 \pm 0.00&
	{\databar{1.00}}	53.59 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	1%
\\
SST                                      & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.18 \pm 0.00&
	{\databar{1.00}}	41.96 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	1%
\\
RRTstar                                  & %
	{\databar{1.00}}	1&
	{\databar{0.01}}	0.59 \pm 0.00&
	{\databar{1.00}}	48.04 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	1%
\\
BFMT                                     & %
	{\databar{1.00}}	1&
	{\databar{0.06}}	2.60 \pm 0.00&
	{\databar{1.00}}	61.97 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	2%
\\
KPIECE1                                  & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.20 \pm 0.00&
	{\databar{1.00}}	174.54 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	8%
\\
SPARStwo                                 & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
RRT                                      & %
	{\databar{1.00}}	1&
	{\databar{0.01}}	0.25 \pm 0.00&
	{\databar{1.00}}	48.58 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	1%
\\
CForest                                  & %
	{\databar{1.00}}	1&
	{\databar{0.01}}	0.36 \pm 0.00&
	{\databar{1.00}}	43.08 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	3%
\\
EST                                      & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	45.00 \pm 0.00&
	{\databar{1.00}}	18.20 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{0.00}}	0%
\\
RRT\#                                    & %
	{\databar{1.00}}	1&
	{\databar{0.02}}	0.85 \pm 0.00&
	{\databar{1.00}}	48.58 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	1%
\\
Theta${}^*$                              & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
PRM                                      & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.01 \pm 0.00&
	{\databar{1.00}}	35.69 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	1%
\\
\rowlabel{\textbf{Steer function: \texttt{POSQ}} (\SI{2.0}{\minute} time limit)}
\\RRT\#                                    & %
	{\databar{1.00}}	1&
	{\databar{0.12}}	14.87 \pm 0.00&
	{\databar{1.00}}	1.61 \pm 0.00&
	{\databar{1.00}}	1.53 \pm 0.00&
	{\databar{1.00}}	1%
\\
SORRTstar                                & %
	{\databar{1.00}}	1&
	{\databar{0.08}}	9.97 \pm 0.00&
	{\databar{1.00}}	1.64 \pm 0.00&
	{\databar{1.00}}	1.60 \pm 0.00&
	{\databar{1.00}}	1%
\\
SPARS                                    & %
	{\databar{1.00}}	1&
	{\databar{0.02}}	1.86 \pm 0.00&
	{\databar{1.00}}	1.58 \pm 0.00&
	{\databar{0.85}}	0.85 \pm 0.00&
	{\databar{1.00}}	4%
\\
CForest                                  & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.32 \pm 0.00&
	{\databar{1.00}}	1.58 \pm 0.00&
	{\databar{1.00}}	1.68 \pm 0.00&
	{\databar{1.00}}	1%
\\
PRM                                      & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.19 \pm 0.00&
	{\databar{1.00}}	1.69 \pm 0.00&
	{\databar{0.81}}	0.81 \pm 0.00&
	{\databar{1.00}}	1%
\\
RRTstar                                  & %
	{\databar{1.00}}	1&
	{\databar{0.12}}	14.64 \pm 0.00&
	{\databar{1.00}}	1.61 \pm 0.00&
	{\databar{1.00}}	1.53 \pm 0.00&
	{\databar{1.00}}	1%
\\
PRMstar                                  & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.17 \pm 0.00&
	{\databar{1.00}}	1.69 \pm 0.00&
	{\databar{0.81}}	0.81 \pm 0.00&
	{\databar{1.00}}	1%
\\
EST                                      & %
	{\databar{1.00}}	1&
	{\databar{0.20}}	24.54 \pm 0.00&
	{\databar{1.00}}	1.73 \pm 0.00&
	{\databar{1.00}}	1.31 \pm 0.00&
	{\databar{1.00}}	10%
\\
SST                                      & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
Theta${}^*$                              & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
PDST                                     & %
	{\databar{1.00}}	1&
	{\databar{0.01}}	0.80 \pm 0.00&
	{\databar{1.00}}	1.72 \pm 0.00&
	{\databar{0.49}}	0.49 \pm 0.00&
	{\databar{1.00}}	1%
\\
RRT                                      & %
	{\databar{1.00}}	1&
	{\databar{0.08}}	10.11 \pm 0.00&
	{\databar{1.00}}	1.39 \pm 0.00&
	{\databar{1.00}}	1.91 \pm 0.00&
	{\databar{1.00}}	27%
\\
BFMT                                     & %
	{\databar{1.00}}	1&
	{\databar{0.15}}	18.27 \pm 0.00&
	{\databar{1.00}}	1.31 \pm 0.00&
	{\databar{1.00}}	1.05 \pm 0.00&
	{\databar{0.00}}	0%
\\
SPARStwo                                 & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.21 \pm 0.00&
	{\databar{1.00}}	1.72 \pm 0.00&
	{\databar{0.34}}	0.34 \pm 0.00&
	{\databar{1.00}}	3%
\\
KPIECE1                                  & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.19 \pm 0.00&
	{\databar{1.00}}	2.55 \pm 0.00&
	{\databar{1.00}}	1.87 \pm 0.00&
	{\databar{1.00}}	16%
\\
kBITstar                                 & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.24 \pm 0.00&
	{\databar{1.00}}	1.55 \pm 0.00&
	{\databar{1.00}}	2.09 \pm 0.00&
	{\databar{1.00}}	4%
\\
InformedRRTstar                          & %
	{\databar{1.00}}	1&
	{\databar{0.06}}	6.78 \pm 0.00&
	{\databar{1.00}}	1.64 \pm 0.00&
	{\databar{1.00}}	1.60 \pm 0.00&
	{\databar{1.00}}	1%
\\
\rowlabel{\textbf{Steer function: \texttt{CC Reeds-Shepp}} (\SI{1.5}{\minute} time limit)}
\\EST                                      & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	90.05 \pm 0.00&
	{\databar{1.00}}	318.21 \pm 0.00&
	{\databar{1.00}}	3.62 \pm 0.00&
	{\databar{1.00}}	20%
\\
kBITstar                                 & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
PDST                                     & %
	{\databar{1.00}}	1&
	{\databar{0.34}}	30.76 \pm 0.00&
	{\databar{1.00}}	272.52 \pm 0.00&
	{\databar{1.00}}	3.00 \pm 0.00&
	{\databar{1.00}}	14%
\\
RRT\#                                    & %
	{\databar{1.00}}	1&
	{\databar{0.78}}	70.04 \pm 0.00&
	{\databar{1.00}}	253.89 \pm 0.00&
	{\databar{1.00}}	3.06 \pm 0.00&
	{\databar{1.00}}	4%
\\
PRMstar                                  & %
	{\databar{1.00}}	1&
	{\databar{0.05}}	4.86 \pm 0.00&
	{\databar{1.00}}	264.98 \pm 0.00&
	{\databar{0.94}}	0.94 \pm 0.00&
	{\databar{1.00}}	8%
\\
PRM                                      & %
	{\databar{1.00}}	1&
	{\databar{0.11}}	10.08 \pm 0.00&
	{\databar{1.00}}	291.57 \pm 0.00&
	{\databar{1.00}}	1.28 \pm 0.00&
	{\databar{1.00}}	25%
\\
KPIECE1                                  & %
	{\databar{1.00}}	1&
	{\databar{0.02}}	1.69 \pm 0.00&
	{\databar{1.00}}	319.84 \pm 0.00&
	{\databar{1.00}}	1.90 \pm 0.00&
	{\databar{1.00}}	30%
\\
SPARStwo                                 & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
Theta${}^*$                              & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
CForest                                  & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	90.34 \pm 0.00&
	{\databar{1.00}}	254.89 \pm 0.00&
	{\databar{1.00}}	3.36 \pm 0.00&
	{\databar{1.00}}	7%
\\
RRT                                      & %
	{\databar{1.00}}	1&
	{\databar{0.40}}	35.97 \pm 0.00&
	{\databar{1.00}}	269.69 \pm 0.00&
	{\databar{0.20}}	0.20 \pm 0.00&
	{\databar{1.00}}	11%
\\
RRTstar                                  & %
	{\databar{1.00}}	1&
	{\databar{0.49}}	44.30 \pm 0.00&
	{\databar{1.00}}	253.89 \pm 0.00&
	{\databar{1.00}}	3.06 \pm 0.00&
	{\databar{1.00}}	4%
\\
InformedRRTstar                          & %
	{\databar{1.00}}	1&
	{\databar{0.02}}	1.65 \pm 0.00&
	{\databar{1.00}}	292.99 \pm 0.00&
	{\databar{0.20}}	0.20 \pm 0.00&
	{\databar{1.00}}	9%
\\
SPARS                                    & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
SORRTstar                                & %
	{\databar{1.00}}	1&
	{\databar{0.46}}	41.59 \pm 0.00&
	{\databar{1.00}}	300.64 \pm 0.00&
	{\databar{0.67}}	0.67 \pm 0.00&
	{\databar{1.00}}	5%
\\
BFMT                                     & %
	{\databar{1.00}}	1&
	{\databar{0.32}}	28.72 \pm 0.00&
	{\databar{1.00}}	238.40 \pm 0.00&
	{\databar{0.23}}	0.23 \pm 0.00&
	{\databar{1.00}}	4%
\\
SST                                      & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	90.02 \pm 0.00&
	{\databar{1.00}}	317.63 \pm 0.00&
	{\databar{0.82}}	0.82 \pm 0.00&
	{\databar{1.00}}	31%
\\
\bottomrule
\end{tabular}

==> table-parking3.tex <==
\begin{tabular}{l*{5}{S[table-format=4.2(6)]}}
\toprule
\bf Planner & \mcc{Solutions Found} & \mcc{Computation Time [s]} & \mcc{Path Length} & \mcc{Maximum Curvature} & \mcc{Cusps} \\\midrule
\rowlabel{\textbf{Steer function: \texttt{Reeds-Shepp}} (\SI{0.2}{\minute} time limit)}
\\kBITstar                                 & %
	{\databar{1.00}}	1&
	{\databar{0.15}}	2.25 \pm 0.00&
	{\databar{1.00}}	28.89 \pm 0.00&
	{\databar{1.00}}	3.40 \pm 0.00&
	{\databar{1.00}}	10%
\\
Theta${}^*$                              & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
RRT                                      & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	15.00 \pm 0.00&
	{\databar{1.00}}	29.59 \pm 0.00&
	{\databar{1.00}}	6.48 \pm 0.00&
	{\databar{1.00}}	13%
\\
KPIECE1                                  & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	15.00 \pm 0.00&
	{\databar{1.00}}	82.81 \pm 0.00&
	{\databar{1.00}}	2.46 \pm 0.00&
	{\databar{1.00}}	34%
\\
CForest                                  & %
	{\databar{1.00}}	1&
	{\databar{0.01}}	0.11 \pm 0.00&
	{\databar{1.00}}	17.27 \pm 0.00&
	{\databar{1.00}}	4.81 \pm 0.00&
	{\databar{1.00}}	6%
\\
SST                                      & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	15.00 \pm 0.00&
	{\databar{1.00}}	15.19 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	5%
\\
EST                                      & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	15.00 \pm 0.00&
	{\databar{1.00}}	40.18 \pm 0.00&
	{\databar{1.00}}	1.96 \pm 0.00&
	{\databar{1.00}}	16%
\\
BFMT                                     & %
	{\databar{1.00}}	1&
	{\databar{0.22}}	3.32 \pm 0.00&
	{\databar{1.00}}	16.02 \pm 0.00&
	{\databar{1.00}}	5.79 \pm 0.00&
	{\databar{1.00}}	6%
\\
InformedRRTstar                          & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	15.00 \pm 0.00&
	{\databar{1.00}}	13.95 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	3%
\\
PRM                                      & %
	{\databar{1.00}}	1&
	{\databar{0.36}}	5.41 \pm 0.00&
	{\databar{1.00}}	19.26 \pm 0.00&
	{\databar{1.00}}	2.96 \pm 0.00&
	{\databar{1.00}}	13%
\\
RRT\#                                    & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	15.06 \pm 0.00&
	{\databar{1.00}}	14.17 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	2%
\\
SPARS                                    & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
RRTstar                                  & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	15.01 \pm 0.00&
	{\databar{1.00}}	11.46 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	1%
\\
PDST                                     & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	15.01 \pm 0.00&
	{\databar{1.00}}	22.78 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	4%
\\
PRMstar                                  & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	15.03 \pm 0.00&
	{\databar{1.00}}	12.52 \pm 0.00&
	{\databar{0.26}}	0.26 \pm 0.00&
	{\databar{1.00}}	3%
\\
SORRTstar                                & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	15.00 \pm 0.00&
	{\databar{1.00}}	13.92 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	3%
\\
SPARStwo                                 & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
\rowlabel{\textbf{Steer function: \texttt{Dubins}} (\SI{0.8}{\minute} time limit)}
\\BFMT                                     & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
kBITstar                                 & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
CForest                                  & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	45.05 \pm 0.00&
	{\databar{1.00}}	89.36 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	3%
\\
KPIECE1                                  & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	45.00 \pm 0.00&
	{\databar{1.00}}	116.49 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	8%
\\
Theta${}^*$                              & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
InformedRRTstar                          & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	45.01 \pm 0.00&
	{\databar{1.00}}	91.81 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	3%
\\
PDST                                     & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	45.01 \pm 0.00&
	{\databar{1.00}}	121.03 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	7%
\\
RRTstar                                  & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	45.02 \pm 0.00&
	{\databar{1.00}}	92.81 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	3%
\\
RRT                                      & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	45.00 \pm 0.00&
	{\databar{1.00}}	98.66 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	3%
\\
PRMstar                                  & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	45.03 \pm 0.00&
	{\databar{1.00}}	138.59 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	5%
\\
EST                                      & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	45.00 \pm 0.00&
	{\databar{1.00}}	109.80 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	12%
\\
SPARS                                    & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
SPARStwo                                 & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
PRM                                      & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	45.04 \pm 0.00&
	{\databar{1.00}}	207.06 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	8%
\\
SORRTstar                                & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	45.00 \pm 0.00&
	{\databar{1.00}}	94.10 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	3%
\\
SST                                      & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	45.00 \pm 0.00&
	{\databar{1.00}}	100.11 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	3%
\\
RRT\#                                    & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	45.00 \pm 0.00&
	{\databar{1.00}}	89.74 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	2%
\\
\rowlabel{\textbf{Steer function: \texttt{POSQ}} (\SI{2.0}{\minute} time limit)}
\\PRMstar                                  & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.55 \pm 0.00&
	{\databar{1.00}}	1.27 \pm 0.00&
	{\databar{1.00}}	1.11 \pm 0.00&
	{\databar{1.00}}	26%
\\
InformedRRTstar                          & %
	{\databar{1.00}}	1&
	{\databar{0.06}}	6.77 \pm 0.00&
	{\databar{1.00}}	1.39 \pm 0.00&
	{\databar{1.00}}	1.05 \pm 0.00&
	{\databar{1.00}}	10%
\\
kBITstar                                 & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.27 \pm 0.00&
	{\databar{1.00}}	1.29 \pm 0.00&
	{\databar{0.38}}	0.38 \pm 0.00&
	{\databar{1.00}}	20%
\\
SPARStwo                                 & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.12 \pm 0.00&
	{\databar{1.00}}	2.40 \pm 0.00&
	{\databar{0.43}}	0.43 \pm 0.00&
	{\databar{1.00}}	12%
\\
RRT                                      & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	120.05 \pm 0.00&
	{\databar{1.00}}	1.80 \pm 0.00&
	{\databar{0.98}}	0.98 \pm 0.00&
	{\databar{1.00}}	13%
\\
Theta${}^*$                              & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
SORRTstar                                & %
	{\databar{1.00}}	1&
	{\databar{0.69}}	83.07 \pm 0.00&
	{\databar{1.00}}	1.50 \pm 0.00&
	{\databar{1.00}}	1.84 \pm 0.00&
	{\databar{1.00}}	16%
\\
CForest                                  & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.13 \pm 0.00&
	{\databar{1.00}}	1.52 \pm 0.00&
	{\databar{1.00}}	1.70 \pm 0.00&
	{\databar{1.00}}	26%
\\
PDST                                     & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.04 \pm 0.00&
	{\databar{1.00}}	1.52 \pm 0.00&
	{\databar{1.00}}	1.46 \pm 0.00&
	{\databar{1.00}}	20%
\\
BFMT                                     & %
	{\databar{1.00}}	1&
	{\databar{0.25}}	30.50 \pm 0.00&
	{\databar{1.00}}	1.41 \pm 0.00&
	{\databar{0.53}}	0.53 \pm 0.00&
	{\databar{1.00}}	5%
\\
SPARS                                    & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.22 \pm 0.00&
	{\databar{1.00}}	1.36 \pm 0.00&
	{\databar{0.42}}	0.42 \pm 0.00&
	{\databar{1.00}}	26%
\\
RRTstar                                  & %
	{\databar{1.00}}	1&
	{\databar{0.92}}	110.86 \pm 0.00&
	{\databar{1.00}}	1.48 \pm 0.00&
	{\databar{1.00}}	1.66 \pm 0.00&
	{\databar{1.00}}	17%
\\
EST                                      & %
	{\databar{1.00}}	1&
	{\databar{0.11}}	13.26 \pm 0.00&
	{\databar{1.00}}	2.31 \pm 0.00&
	{\databar{0.78}}	0.78 \pm 0.00&
	{\databar{1.00}}	9%
\\
PRM                                      & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.51 \pm 0.00&
	{\databar{1.00}}	1.64 \pm 0.00&
	{\databar{1.00}}	1.74 \pm 0.00&
	{\databar{1.00}}	11%
\\
SST                                      & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
KPIECE1                                  & %
	{\databar{1.00}}	1&
	{\databar{0.00}}	0.09 \pm 0.00&
	{\databar{1.00}}	2.97 \pm 0.00&
	{\databar{1.00}}	2.81 \pm 0.00&
	{\databar{1.00}}	22%
\\
RRT\#                                    & %
	{\databar{1.00}}	1&
	{\databar{0.97}}	116.70 \pm 0.00&
	{\databar{1.00}}	1.48 \pm 0.00&
	{\databar{1.00}}	1.66 \pm 0.00&
	{\databar{1.00}}	17%
\\
\rowlabel{\textbf{Steer function: \texttt{CC Reeds-Shepp}} (\SI{1.5}{\minute} time limit)}
\\InformedRRTstar                          & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	90.09 \pm 0.00&
	{\databar{1.00}}	266.57 \pm 0.00&
	{\databar{0.20}}	0.20 \pm 0.00&
	{\databar{1.00}}	4%
\\
PDST                                     & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	90.01 \pm 0.00&
	{\databar{1.00}}	296.39 \pm 0.00&
	{\databar{0.29}}	0.29 \pm 0.00&
	{\databar{1.00}}	9%
\\
RRTstar                                  & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	90.01 \pm 0.00&
	{\databar{1.00}}	271.00 \pm 0.00&
	{\databar{0.20}}	0.20 \pm 0.00&
	{\databar{1.00}}	4%
\\
PRMstar                                  & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	90.17 \pm 0.00&
	{\databar{1.00}}	193.39 \pm 0.00&
	{\databar{0.19}}	0.19 \pm 0.00&
	{\databar{1.00}}	4%
\\
SORRTstar                                & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	90.00 \pm 0.00&
	{\databar{1.00}}	259.00 \pm 0.00&
	{\databar{0.20}}	0.20 \pm 0.00&
	{\databar{1.00}}	4%
\\
PRM                                      & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	90.48 \pm 0.00&
	{\databar{1.00}}	232.52 \pm 0.00&
	{\databar{0.17}}	0.17 \pm 0.00&
	{\databar{1.00}}	4%
\\
SPARS                                    & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
Theta${}^*$                              & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
SPARStwo                                 & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
BFMT                                     & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
kBITstar                                 & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
EST                                      & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	90.01 \pm 0.00&
	{\databar{1.00}}	322.13 \pm 0.00&
	{\databar{1.00}}	2.06 \pm 0.00&
	{\databar{1.00}}	23%
\\
KPIECE1                                  & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	90.00 \pm 0.00&
	{\databar{1.00}}	504.61 \pm 0.00&
	{\databar{1.00}}	1.30 \pm 0.00&
	{\databar{1.00}}	76%
\\
RRT                                      & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	90.01 \pm 0.00&
	{\databar{1.00}}	172.88 \pm 0.00&
	{\databar{0.54}}	0.54 \pm 0.00&
	{\databar{1.00}}	7%
\\
RRT\#                                    & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	90.00 \pm 0.00&
	{\databar{1.00}}	318.75 \pm 0.00&
	{\databar{0.20}}	0.20 \pm 0.00&
	{\databar{1.00}}	4%
\\
SST                                      & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	90.00 \pm 0.00&
	{\databar{1.00}}	301.68 \pm 0.00&
	{\databar{0.20}}	0.20 \pm 0.00&
	{\databar{1.00}}	17%
\\
CForest                                  & %
	{\databar{1.00}}	1&
	{\databar{0.02}}	1.39 \pm 0.00&
	{\databar{1.00}}	331.11 \pm 0.00&
	{\databar{0.20}}	0.20 \pm 0.00&
	{\databar{1.00}}	3%
\\
\bottomrule
\end{tabular}

==> table-warehouse.tex <==
\begin{tabular}{l*{5}{S[table-format=4.2(6)]}}
\toprule
\bf Planner & \mcc{Solutions Found} & \mcc{Computation Time [s]} & \mcc{Path Length} & \mcc{Maximum Curvature} & \mcc{Cusps} \\\midrule
\rowlabel{\textbf{Steer function: \texttt{Reeds-Shepp}} (\SI{0.2}{\minute} time limit)}
\\Theta${}^*$                              & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
EST                                      & %
	{\databar{1.00}}	1&
	{\databar{0.25}}	3.75 \pm 0.00&
	{\databar{1.00}}	227.91 \pm 0.00&
	{\databar{0.88}}	0.88 \pm 0.00&
	{\databar{1.00}}	15%
\\
PDST                                     & %
	{\databar{1.00}}	1&
	{\databar{0.12}}	1.80 \pm 0.00&
	{\databar{1.00}}	245.13 \pm 0.00&
	{\databar{0.93}}	0.93 \pm 0.00&
	{\databar{1.00}}	18%
\\
SPARS                                    & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	15.16 \pm 0.00&
	{\databar{1.00}}	240.64 \pm 0.00&
	{\databar{0.86}}	0.86 \pm 0.00&
	{\databar{1.00}}	12%
\\
kBITstar                                 & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	15.01 \pm 0.00&
	{\databar{1.00}}	181.07 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	1%
\\
SST                                      & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	15.00 \pm 0.00&
	{\databar{1.00}}	234.79 \pm 0.00&
	{\databar{0.81}}	0.81 \pm 0.00&
	{\databar{1.00}}	13%
\\
SPARStwo                                 & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	15.01 \pm 0.00&
	{\databar{1.00}}	203.10 \pm 0.00&
	{\databar{1.00}}	1.01 \pm 0.00&
	{\databar{1.00}}	7%
\\
RRTstar                                  & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	15.05 \pm 0.00&
	{\databar{1.00}}	179.18 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	1%
\\
SORRTstar                                & %
	{\databar{1.00}}	1&
	{\databar{0.83}}	12.46 \pm 0.00&
	{\databar{1.00}}	92.64 \pm 0.00&
	{\databar{1.00}}	2.00 \pm 0.00&
	{\databar{1.00}}	6%
\\
PRM                                      & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	15.05 \pm 0.00&
	{\databar{1.00}}	204.57 \pm 0.00&
	{\databar{0.97}}	0.97 \pm 0.00&
	{\databar{1.00}}	8%
\\
RRT                                      & %
	{\databar{1.00}}	1&
	{\databar{0.03}}	0.43 \pm 0.00&
	{\databar{1.00}}	202.14 \pm 0.00&
	{\databar{0.97}}	0.97 \pm 0.00&
	{\databar{1.00}}	4%
\\
KPIECE1                                  & %
	{\databar{1.00}}	1&
	{\databar{0.13}}	1.92 \pm 0.00&
	{\databar{1.00}}	367.83 \pm 0.00&
	{\databar{0.56}}	0.56 \pm 0.00&
	{\databar{1.00}}	39%
\\
PRMstar                                  & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	15.06 \pm 0.00&
	{\databar{1.00}}	192.93 \pm 0.00&
	{\databar{0.98}}	0.98 \pm 0.00&
	{\databar{1.00}}	4%
\\
CForest                                  & %
	{\databar{1.00}}	1&
	{\databar{0.60}}	9.01 \pm 0.00&
	{\databar{1.00}}	99.42 \pm 0.00&
	{\databar{1.00}}	1.14 \pm 0.00&
	{\databar{1.00}}	4%
\\
RRT\#                                    & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	15.02 \pm 0.00&
	{\databar{1.00}}	179.88 \pm 0.00&
	{\databar{0.45}}	0.45 \pm 0.00&
	{\databar{1.00}}	1%
\\
BFMT                                     & %
	{\databar{1.00}}	1&
	{\databar{0.25}}	3.81 \pm 0.00&
	{\databar{1.00}}	86.90 \pm 0.00&
	{\databar{0.51}}	0.51 \pm 0.00&
	{\databar{1.00}}	3%
\\
InformedRRTstar                          & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	15.03 \pm 0.00&
	{\databar{1.00}}	176.93 \pm 0.00&
	{\databar{0.18}}	0.18 \pm 0.00&
	{\databar{1.00}}	1%
\\
\rowlabel{\textbf{Steer function: \texttt{Dubins}} (\SI{0.8}{\minute} time limit)}
\\BFMT                                     & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
InformedRRTstar                          & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	45.04 \pm 0.00&
	{\databar{1.00}}	177.78 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	1%
\\
PDST                                     & %
	{\databar{1.00}}	1&
	{\databar{0.02}}	0.91 \pm 0.00&
	{\databar{1.00}}	177.51 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	1%
\\
SPARStwo                                 & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
RRTstar                                  & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	45.02 \pm 0.00&
	{\databar{1.00}}	175.38 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	1%
\\
SST                                      & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	45.00 \pm 0.00&
	{\databar{1.00}}	181.97 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	1%
\\
KPIECE1                                  & %
	{\databar{1.00}}	1&
	{\databar{0.40}}	17.95 \pm 0.00&
	{\databar{1.00}}	193.21 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	1%
\\
kBITstar                                 & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	45.00 \pm 0.00&
	{\databar{1.00}}	170.00 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	1%
\\
CForest                                  & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	45.17 \pm 0.00&
	{\databar{1.00}}	174.56 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	1%
\\
SPARS                                    & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
RRT\#                                    & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	45.02 \pm 0.00&
	{\databar{1.00}}	180.03 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	1%
\\
PRMstar                                  & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	45.16 \pm 0.00&
	{\databar{1.00}}	252.74 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	8%
\\
RRT                                      & %
	{\databar{1.00}}	1&
	{\databar{0.01}}	0.47 \pm 0.00&
	{\databar{1.00}}	180.03 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	1%
\\
EST                                      & %
	{\databar{1.00}}	1&
	{\databar{0.05}}	2.08 \pm 0.00&
	{\databar{1.00}}	187.73 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	1%
\\
SORRTstar                                & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	45.15 \pm 0.00&
	{\databar{1.00}}	179.15 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	1%
\\
PRM                                      & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	45.02 \pm 0.00&
	{\databar{1.00}}	204.47 \pm 0.00&
	{\databar{0.25}}	0.25 \pm 0.00&
	{\databar{1.00}}	2%
\\
\rowlabel{\textbf{Steer function: \texttt{POSQ}} (\SI{2.0}{\minute} time limit)}
\\SORRTstar                                & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	120.02 \pm 0.00&
	{\databar{1.00}}	4.87 \pm 0.00&
	{\databar{0.99}}	0.99 \pm 0.00&
	{\databar{1.00}}	1%
\\
SPARS                                    & %
	{\databar{1.00}}	1&
	{\databar{0.07}}	8.09 \pm 0.00&
	{\databar{1.00}}	5.91 \pm 0.00&
	{\databar{1.00}}	1.05 \pm 0.00&
	{\databar{1.00}}	13%
\\
PRM                                      & %
	{\databar{1.00}}	1&
	{\databar{0.07}}	8.13 \pm 0.00&
	{\databar{1.00}}	5.96 \pm 0.00&
	{\databar{0.60}}	0.60 \pm 0.00&
	{\databar{1.00}}	9%
\\
KPIECE1                                  & %
	{\databar{1.00}}	1&
	{\databar{0.05}}	5.79 \pm 0.00&
	{\databar{1.00}}	7.14 \pm 0.00&
	{\databar{0.60}}	0.60 \pm 0.00&
	{\databar{1.00}}	42%
\\
SPARStwo                                 & %
	{\databar{1.00}}	1&
	{\databar{0.07}}	8.14 \pm 0.00&
	{\databar{1.00}}	6.31 \pm 0.00&
	{\databar{1.00}}	1.35 \pm 0.00&
	{\databar{1.00}}	2%
\\
PRMstar                                  & %
	{\databar{1.00}}	1&
	{\databar{0.02}}	2.58 \pm 0.00&
	{\databar{1.00}}	6.99 \pm 0.00&
	{\databar{0.61}}	0.61 \pm 0.00&
	{\databar{1.00}}	10%
\\
BFMT                                     & %
	{\databar{1.00}}	1&
	{\databar{0.92}}	109.96 \pm 0.00&
	{\databar{1.00}}	3.81 \pm 0.00&
	{\databar{1.00}}	1.30 \pm 0.00&
	{\databar{1.00}}	14%
\\
PDST                                     & %
	{\databar{1.00}}	1&
	{\databar{0.05}}	6.42 \pm 0.00&
	{\databar{1.00}}	5.13 \pm 0.00&
	{\databar{0.97}}	0.97 \pm 0.00&
	{\databar{1.00}}	19%
\\
EST                                      & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	120.00 \pm 0.00&
	{\databar{1.00}}	2.30 \pm 0.00&
	{\databar{1.00}}	1.73 \pm 0.00&
	{\databar{1.00}}	19%
\\
RRT\#                                    & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	120.03 \pm 0.00&
	{\databar{1.00}}	6.17 \pm 0.00&
	{\databar{0.38}}	0.38 \pm 0.00&
	{\databar{1.00}}	2%
\\
InformedRRTstar                          & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	120.01 \pm 0.00&
	{\databar{1.00}}	4.87 \pm 0.00&
	{\databar{0.99}}	0.99 \pm 0.00&
	{\databar{1.00}}	1%
\\
CForest                                  & %
	{\databar{1.00}}	1&
	{\databar{0.17}}	20.40 \pm 0.00&
	{\databar{1.00}}	6.58 \pm 0.00&
	{\databar{0.46}}	0.46 \pm 0.00&
	{\databar{1.00}}	2%
\\
RRT                                      & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	120.00 \pm 0.00&
	{\databar{1.00}}	2.66 \pm 0.00&
	{\databar{0.17}}	0.17 \pm 0.00&
	{\databar{1.00}}	15%
\\
RRTstar                                  & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	120.03 \pm 0.00&
	{\databar{1.00}}	6.17 \pm 0.00&
	{\databar{0.38}}	0.38 \pm 0.00&
	{\databar{1.00}}	2%
\\
SST                                      & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
kBITstar                                 & %
	{\databar{1.00}}	1&
	{\databar{0.18}}	21.21 \pm 0.00&
	{\databar{1.00}}	5.97 \pm 0.00&
	{\databar{0.60}}	0.60 \pm 0.00&
	{\databar{1.00}}	19%
\\
\rowlabel{\textbf{Steer function: \texttt{CC Reeds-Shepp}} (\SI{1.5}{\minute} time limit)}
\\RRT                                      & %
	{\databar{1.00}}	1&
	{\databar{0.42}}	37.61 \pm 0.00&
	{\databar{1.00}}	377.03 \pm 0.00&
	{\databar{0.74}}	0.74 \pm 0.00&
	{\databar{1.00}}	19%
\\
SPARStwo                                 & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
kBITstar                                 & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	90.01 \pm 0.00&
	{\databar{1.00}}	310.85 \pm 0.00&
	{\databar{0.20}}	0.20 \pm 0.00&
	{\databar{1.00}}	1%
\\
KPIECE1                                  & %
	{\databar{1.00}}	1&
	{\databar{0.30}}	26.94 \pm 0.00&
	{\databar{1.00}}	859.09 \pm 0.00&
	{\databar{1.00}}	1.05 \pm 0.00&
	{\databar{1.00}}	73%
\\
InformedRRTstar                          & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	90.01 \pm 0.00&
	{\databar{1.00}}	318.66 \pm 0.00&
	{\databar{0.69}}	0.69 \pm 0.00&
	{\databar{1.00}}	3%
\\
SPARS                                    & %
	0 &
	N / A&
	N / A&
	N / A&
	N / A%
\\
RRTstar                                  & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	90.24 \pm 0.00&
	{\databar{1.00}}	272.83 \pm 0.00&
	{\databar{0.20}}	0.20 \pm 0.00&
	{\databar{1.00}}	1%
\\
SST                                      & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	90.04 \pm 0.00&
	{\databar{1.00}}	447.07 \pm 0.00&
	{\databar{0.43}}	0.43 \pm 0.00&
	{\databar{1.00}}	25%
\\
PDST                                     & %
	{\databar{1.00}}	1&
	{\databar{0.48}}	43.22 \pm 0.00&
	{\databar{1.00}}	330.84 \pm 0.00&
	{\databar{0.29}}	0.29 \pm 0.00&
	{\databar{1.00}}	15%
\\
PRMstar                                  & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	90.14 \pm 0.00&
	{\databar{1.00}}	266.69 \pm 0.00&
	{\databar{0.79}}	0.79 \pm 0.00&
	{\databar{1.00}}	5%
\\
PRM                                      & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	90.09 \pm 0.00&
	{\databar{1.00}}	348.59 \pm 0.00&
	{\databar{0.85}}	0.85 \pm 0.00&
	{\databar{1.00}}	11%
\\
EST                                      & %
	{\databar{1.00}}	1&
	{\databar{0.72}}	64.81 \pm 0.00&
	{\databar{1.00}}	656.53 \pm 0.00&
	{\databar{1.00}}	1.33 \pm 0.00&
	{\databar{1.00}}	53%
\\
BFMT                                     & %
	{\databar{1.00}}	1&
	{\databar{0.35}}	31.12 \pm 0.00&
	{\databar{1.00}}	266.46 \pm 0.00&
	{\databar{1.00}}	1.86 \pm 0.00&
	{\databar{1.00}}	8%
\\
SORRTstar                                & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	90.15 \pm 0.00&
	{\databar{1.00}}	296.84 \pm 0.00&
	{\databar{1.00}}	1.43 \pm 0.00&
	{\databar{1.00}}	5%
\\
CForest                                  & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	90.46 \pm 0.00&
	{\databar{1.00}}	320.26 \pm 0.00&
	{\databar{0.88}}	0.88 \pm 0.00&
	{\databar{1.00}}	5%
\\
RRT\#                                    & %
	{\databar{1.00}}	1&
	{\databar{1.00}}	90.11 \pm 0.00&
	{\databar{1.00}}	244.34 \pm 0.00&
	{\databar{0.20}}	0.20 \pm 0.00&
	{\databar{1.00}}	1%
\\
\bottomrule
\end{tabular}
